Likelihood-Free Inference with Generative Neural Networks via Scoring Rule Minimization

Bayesian Likelihood-Free Inference methods yield posterior approximations for simulator models with intractable likelihood. Recently, many works trained neural networks to approximate either the intractable likelihood or the posterior directly. Most proposals use normalizing flows, namely neural networks parametrizing invertible maps used to transform samples from an underlying base measure; the probability density of the transformed samples is then accessible and the normalizing flow can be trained via maximum likelihood on simulated parameter-observation pairs. A recent work [Ramesh et al., 2022] approximated instead the posterior with generative networks, which drop the invertibility requirement and are thus a more flexible class of distributions scaling to high-dimensional and structured data. However, generative networks only allow sampling from the parametrized distribution; for this reason, Ramesh et al. [2022] follows the common solution of adversarial training, where the generative network plays a min-max game against a "critic" network. This procedure is unstable and can lead to a learned distribution underestimating the uncertainty - in extreme cases collapsing to a single point. Here, we propose to approximate the posterior with generative networks trained by Scoring Rule minimization, an overlooked adversarial-free method enabling smooth training and better uncertainty quantification. In simulation studies, the Scoring Rule approach yields better performances with shorter training time with respect to the adversarial framework.

==> tables/camera_model_all_metrics_n_gen=10 <==
\begin{tabular}{llllrr}
\hline
                         & RMSE $ \downarrow $   & Cal. Err. $ \downarrow $   & R$^2$ $ \uparrow $    &   Runtime (sec) &   Early stopping epoch \\
\hline
 GAN 
 0.25 $\pm$ 0.19       & 0.50 $\pm$ 0.00            & -23.94 $\pm$ 366.08   &           45398 &                   3600 \\
 Energy              & 0.08 $\pm$ 0.05       & 0.36 $\pm$ 0.12            & -24.39 $\pm$ 450.13   &           24555 &                   4200 \\
 Energy patched 5 8  & 0.06 $\pm$ 0.05       & 0.36 $\pm$ 0.12            & -2.14 $\pm$ 55.86     &           22633 &                   4000 \\
 Energy patched 7 14 & 0.07 $\pm$ 0.05       & 0.37 $\pm$ 0.12            & -10.33 $\pm$ 227.38   &           24033 &                   3600 \\
 Kernel              & 0.06 $\pm$ 0.05       & 0.32 $\pm$ 0.15            & -7.22 $\pm$ 164.26    &           21862 &                   3200 \\
 Kernel patched 5 8  & 0.07 $\pm$ 0.05       & 0.36 $\pm$ 0.12            & -10.29 $\pm$ 222.12   &           22545 &                   3200 \\
 Kernel patched 7 14 & 0.10 $\pm$ 0.06       & 0.38 $\pm$ 0.11            & -144.56 $\pm$ 2952.80 &           20605 &                   3600 \\
\hline
\end{tabular}

==> tables/camera_model_best_methods_all_metrics_n_gen=10 <==
\begin{tabular}{lcccrr}
\hline
                        & RMSE $ \downarrow $   & Cal. Err. $ \downarrow $   & R$^2$ $ \uparrow $   &   Runtime (sec) &   Early stopping epoch \\
\hline
 GAN              & 0.25 $\pm$ 0.19       & 0.50 $\pm$ 0.00            & -23.94 $\pm$ 366.08  &           45,398 &                   3,600 \\
 Energy   & 0.06 $\pm$ 0.05       & 0.36 $\pm$ 0.12            & -2.14 $\pm$ 55.86    &           22,633 &                   4,000 \\
 Kernel   & 0.07 $\pm$ 0.05       & 0.36 $\pm$ 0.12            & -10.29 $\pm$ 222.12  &           22,545 &                   3,200 \\
\hline
\end{tabular}

==> tables/slcp_all_metrics_n_gen=20 <==
\begin{tabular}{llllllllll}
\hline
                          & GAN 1000        & GAN 10000       & GAN 100000      & Energy 1000     & Energy 10000    & Energy 100000   & Kernel 1000     & Kernel 10000    & Kernel 100000   \\
\hline
 C2ST $ \downarrow $      & 0.97 $\pm$ 0.02 & 0.94 $\pm$ 0.03 & 0.92 $\pm$ 0.03 & 0.99 $\pm$ 0.01 & 0.98 $\pm$ 0.01 & 0.95 $\pm$ 0.02 & 0.99 $\pm$ 0.01 & 0.99 $\pm$ 0.01 & 0.98 $\pm$ 0.01 \\
 RMSE $ \downarrow $      & 0.24 $\pm$ 0.05 & 0.23 $\pm$ 0.05 & 0.23 $\pm$ 0.05 & 0.25 $\pm$ 0.06 & 0.23 $\pm$ 0.05 & 0.22 $\pm$ 0.06 & 0.25 $\pm$ 0.05 & 0.23 $\pm$ 0.05 & 0.22 $\pm$ 0.06 \\
 Cal. Err. $ \downarrow $ & 0.13 $\pm$ 0.05 & 0.08 $\pm$ 0.03 & 0.06 $\pm$ 0.03 & 0.22 $\pm$ 0.07 & 0.10 $\pm$ 0.07 & 0.07 $\pm$ 0.04 & 0.24 $\pm$ 0.08 & 0.16 $\pm$ 0.10 & 0.13 $\pm$ 0.10 \\
 R$^2$ $ \uparrow $       & 0.25 $\pm$ 0.29 & 0.35 $\pm$ 0.30 & 0.35 $\pm$ 0.30 & 0.18 $\pm$ 0.35 & 0.34 $\pm$ 0.31 & 0.38 $\pm$ 0.32 & 0.23 $\pm$ 0.31 & 0.34 $\pm$ 0.30 & 0.37 $\pm$ 0.31 \\
 Runtime (sec)            & 4796            & 9671            & 30963           & 885             & 720             & 1645            & 1330            & 697             & 1210            \\
 Early stopping epoch     & 20000           & 20000           & 20000           & 1100            & 1100            & 2100            & 1000            & 1000            & 1200            \\
\hline
\end{tabular}

==> tables/two_moons_all_metrics_n_gen=20 <==
\begin{tabular}{llllllllll}
\hline
                          & GAN 1000        & GAN 10000       & GAN 100000      & Energy 1000     & Energy 10000    & Energy 100000   & Kernel 1000     & Kernel 10000    & Kernel 100000   \\
\hline
 C2ST $ \downarrow $      & 0.85 $\pm$ 0.05 & 0.81 $\pm$ 0.03 & 0.82 $\pm$ 0.07 & 0.85 $\pm$ 0.04 & 0.74 $\pm$ 0.07 & 0.73 $\pm$ 0.04 & 0.96 $\pm$ 0.02 & 0.93 $\pm$ 0.01 & 0.92 $\pm$ 0.02 \\
 RMSE $ \downarrow $      & 0.20 $\pm$ 0.00 & 0.20 $\pm$ 0.00 & 0.20 $\pm$ 0.00 & 0.20 $\pm$ 0.00 & 0.20 $\pm$ 0.00 & 0.20 $\pm$ 0.00 & 0.20 $\pm$ 0.00 & 0.20 $\pm$ 0.00 & 0.20 $\pm$ 0.00 \\
 Cal. Err. $ \downarrow $ & 0.07 $\pm$ 0.01 & 0.06 $\pm$ 0.01 & 0.07 $\pm$ 0.02 & 0.06 $\pm$ 0.00 & 0.03 $\pm$ 0.01 & 0.03 $\pm$ 0.00 & 0.12 $\pm$ 0.01 & 0.03 $\pm$ 0.01 & 0.03 $\pm$ 0.01 \\
 R$^2$ $ \uparrow $       & 0.50 $\pm$ 0.01 & 0.49 $\pm$ 0.01 & 0.51 $\pm$ 0.01 & 0.51 $\pm$ 0.01 & 0.51 $\pm$ 0.01 & 0.51 $\pm$ 0.01 & 0.49 $\pm$ 0.01 & 0.50 $\pm$ 0.01 & 0.50 $\pm$ 0.01 \\
 Runtime (sec)            & 4799            & 8163            & 30232           & 896             & 3228            & 10805           & 852             & 3267            & 10902           \\
 Early stopping epoch     & 20000           & 20000           & 20000           & 20000           & 20000           & 20000           & 20000           & 20000           & 20000           \\
\hline
\end{tabular}
